Jointly Trained Sequential Labeling and Classification by Sparse Attention Neural Networks

Sentence-level classification and sequential labeling are two fundamental tasks in language understanding. While these two tasks are usually modeled separately, in reality, they are often correlated, for example in intent classification and slot filling, or in topic classification and named-entity recognition. In order to utilize the potential benefits from their correlations, we propose a jointly trained model for learning the two tasks simultaneously via Long Short-Term Memory (LSTM) networks. This model predicts the sentence-level category and the word-level label sequence from the stepwise output hidden representations of LSTM. We also introduce a novel mechanism of "sparse attention" to weigh words differently based on their semantic relevance to sentence-level classification. The proposed method outperforms baseline models on ATIS and TREC datasets.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
#figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	#@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "15 15 15 15" main.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

